On the dangers of partial diagrammatic summations: Benchmarks for the two-dimensional Hubbard model in the weak-coupling regime

We study the two-dimensional Hubbard model in the weak-coupling regime and compare the self-energy obtained from various approximate diagrammatic schemes to the result of diagrammatic Monte Carlo simulations, which sum up all weak-coupling diagrams up to a given order. While dynamical mean-field theory provides a good approximation for the local part of the self-energy, including its frequency dependence, the partial summation of bubble and/or ladder diagrams typically yields worse results than second order perturbation theory. Even widely used self-consistent schemes such as GW or the fluctuation-exchange approximation (FLEX) are found to be unreliable. Combining the dynamical mean-field self-energy with the nonlocal component of GW in GW+DMFT yields improved results for the local self-energy and nonlocal self-energies of the correct order of magnitude, but here, too, a more reliable scheme is obtained by restricting the nonlocal contribution to the second order diagram. FLEX+DMFT is found to give accurate results in the low-density regime, but even worse results than FLEX near half-filling.

==> diagmcdiags.tex <==
\beginpgfgraphicnamed{diagmc}
\begin{minipage}{\columnwidth}
\begin{align*}
(a) \quad &
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[right = of v1] (v2);
\coordinate[right = of v2] (v3);
\coordinate[vertex, right = of v3] (v4);
\coordinate[vertex, below = of v4] (v5);
\coordinate[vertex, below = of v1] (v8);
\coordinate[vertex, above =0.25\distance of v2] (v6);
\coordinate[vertex, above =0.25\distance of v3] (v7);
\coordinate[vertex, above = of v6] (v6a);
\coordinate[vertex, above = of v7] (v7a);
\draw[photon](v1) -- (v8);
\draw[photon](v4) -- (v5);
\draw[photon](v6) -- (v6a);
\draw[photon](v7) -- (v7a);
\draw[fermion] (v8) -- (v5);
\draw[fermion] (v1) to[out = 20, in = 160] (v4);
\draw[fermion] (v4) to[out = 200, in = 340] (v1);
\draw[fermion] (v6a) to[out = 20, in = 160] (v7a);
\draw[fermion] (v7a) to[out = 200, in = 340] (v6a);
\end{tikzpicture}
}
+
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[right = of v1] (v2);
\coordinate[right = of v2] (v3);
\coordinate[vertex, right = of v3] (v4);
\coordinate[vertex, below = of v4] (v5);
\coordinate[vertex, below = of v1] (v8);
\coordinate[vertex, left = of v5] (v6);
\coordinate[vertex, right = of v8] (v7);
\coordinate[vertex, above =0.4\distance of v6] (v6a);
\coordinate[vertex, above =0.4\distance of v7] (v7a);
\draw[photon](v1) -- (v8);
\draw[photon](v4) -- (v5);
\draw[photon](v6) -- (v6a);
\draw[photon](v7) -- (v7a);
\draw[fermion] (v8) -- (v5);
\draw[fermion] (v1) to[out = 20, in = 160] (v4);
\draw[fermion] (v4) to[out = 200, in = 340] (v1);
\draw[fermion] (v7a) to[out = 20, in = 160] (v6a);
\draw[fermion] (v6a) to[out = 200, in = 340] (v7a);
\end{tikzpicture}
}
+ \cdots
\\
(b) \quad &
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, right = of v2] (v3);
\coordinate[vertex, right = of v3] (v4);
\coordinate[vertex, below = of v4] (v5);
\coordinate[vertex, below = of v3] (v6);
\coordinate[vertex, below = of v2] (v7);
\coordinate[vertex, below = of v1] (v8);
\draw[photon](v1) -- (v8);
\draw[photon](v2) -- (v7);
\draw[photon](v3) -- (v5);
\draw[photon](v4) -- (v6);
\draw[fermion] (v2) -- (v1);
\draw[fermion] (v3) -- (v2);
\draw[fermion] (v4) -- (v3);
\draw[fermion] (v6) -- (v5);
\draw[fermion] (v7) -- (v6);
\draw[fermion] (v8) -- (v7);
\draw[fermion] (v1) to[out = 60, in = 120] (v4);
\end{tikzpicture}
}
+
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, right = of v2] (v3);
\coordinate[vertex, right = of v3] (v4);
\coordinate[vertex, below = of v4] (v5);
\coordinate[vertex, below = of v3] (v6);
\coordinate[vertex, below = of v2] (v7);
\coordinate[vertex, below = of v1] (v8);
\draw[photon](v1) -- (v8);
\draw[photon](v2) -- (v6);
\draw[photon](v3) -- (v7);
\draw[photon](v4) -- (v5);
\draw[fermion] (v2) -- (v1);
\draw[fermion] (v3) -- (v2);
\draw[fermion] (v4) -- (v3);
\draw[fermion] (v6) -- (v5);
\draw[fermion] (v7) -- (v6);
\draw[fermion] (v8) -- (v7);
\draw[fermion] (v1) to[out = 60, in = 120] (v4);
\end{tikzpicture}
}
+\\
&
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, right = of v2] (v3);
\coordinate[vertex, right = of v3] (v4);
\coordinate[vertex, below = of v4] (v5);
\coordinate[vertex, below = of v3] (v6);
\coordinate[vertex, below = of v2] (v7);
\coordinate[vertex, below = of v1] (v8);
\draw[photon](v1) -- (v8);
\draw[photon](v2) -- (v5);
\draw[photon](v3) -- (v7);
\draw[photon](v4) -- (v6);
\draw[fermion] (v2) -- (v1);
\draw[fermion] (v3) -- (v2);
\draw[fermion] (v4) -- (v3);
\draw[fermion] (v6) -- (v5);
\draw[fermion] (v7) -- (v6);
\draw[fermion] (v8) -- (v7);
\draw[fermion] (v1) to[out = 60, in = 120] (v4);
\end{tikzpicture}
}
+ \cdots
\\
(c) \quad &
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, right = of v2] (v3);
\coordinate[vertex, right = of v3] (v4);
\coordinate[vertex, below = of v4] (v5);
\coordinate[vertex, below = of v3] (v6);
\coordinate[vertex, below = of v2] (v7);
\coordinate[vertex, below = of v1] (v8);
\draw[photon](v1) -- (v8);
\draw[photon](v4) -- (v5);
\draw[photon](v2) -- (v6);
\draw[photon](v3) -- (v7);
\draw[fermion] (v6) -- (v5);
\draw[fermion] (v7) -- (v6);
\draw[fermion] (v8) -- (v7);
\draw[fermion] (v1) to[out = 60, in = 120] (v2);
\draw[fermion] (v2) to[out = 240, in = 300] (v1);
\draw[fermion] (v3) to[out = 60, in = 120] (v4);
\draw[fermion] (v4) to[out = 240, in = 300] (v3);
\end{tikzpicture}
}
+
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, right = of v2] (v3);
\coordinate[vertex, right = of v3] (v4);
\coordinate[vertex, below = of v4] (v5);
\coordinate[vertex, below =0.85\distance of v2] (v6);
\coordinate[vertex, above =0.85\distance of v3] (v7);
\coordinate[vertex, below = of v1] (v8);
\draw[photon](v1) -- (v8);
\draw[photon](v4) -- (v5);
\draw[photon](v2) -- (v6);
\draw[photon](v3) -- (v7);
\draw[fermion] (v8) -- (v5);
\draw[fermion] (v1) to[out = 60, in = 120] (v4);
\draw[fermion] (v4) to[out = 240, in = 300] (v1);
\draw[fermion] (v2) to[out = 60, in = 120] (v3);
\draw[fermion] (v3) to[out = 240, in = 300] (v2);
\end{tikzpicture}
}
+ \cdots
\end{align*}
\end{minipage}
\endpgfgraphicnamed


==> mbptdiags.tex <==
\beginpgfgraphicnamed{mbpt}
\begin{minipage}{\columnwidth}
\begin{align*}
\Sigma^{(2)} =
\scalebox{.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[below = of v1](f1);
\draw[photon](v1) -- (f1);
\draw[fermion] (v1) arc (-90:270:0.6cm);
\end{tikzpicture}
}
+&
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, below = of v2] (v3);
\coordinate[vertex, left = of v3] (v4);
\draw[photon](v1) -- (v4);
\draw[photon](v2) -- (v3);
\draw[fermion] (v4) -- (v3);
\draw[fermion] (v1) to [out = 60, in = 120] (v2);
\draw[fermion] (v2) to [out = 240, in = 300] (v1);
\end{tikzpicture}
}
\\
\Sigma_{\text{SGW}} =
\scalebox{.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[below = of v1](f1);
\draw[photon](v1) -- (f1);
\draw[fermion] (v1) arc (-90:270:0.6cm);
\end{tikzpicture}
}
+&
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, below = of v2] (v3);
\coordinate[vertex, left = of v3] (v4);
\draw[photon](v1) -- (v4);
\draw[photon](v2) -- (v3);
\draw[fermion] (v4) -- (v3);
\draw[fermion] (v1) to [out = 60, in = 120] (v2);
\draw[fermion] (v2) to [out = 240, in = 300] (v1);
\end{tikzpicture}
}
+
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, above = of v2] (v3);
\coordinate[vertex, right = of v3] (v4);
\coordinate[vertex, below = of v4] (v5);
\coordinate[vertex, right = of v5] (v6);
\coordinate[vertex, below = of v6] (v7);
\coordinate[vertex, below = of v1] (v8);
\draw[photon](v1) -- (v8);
\draw[photon](v2) -- (v3);
\draw[photon](v4) -- (v5);
\draw[photon](v6) -- (v7);
\draw[fermion] (v8) -- (v7);
\draw[fermion] (v1) to[out = 60, in = 120] (v2);
\draw[fermion] (v2) to[out = 240, in = 300] (v1);
\draw[fermion] (v3) to[out = 60, in = 120] (v4);
\draw[fermion] (v4) to[out = 240, in = 300] (v3);
\draw[fermion] (v5) to[out = 60, in = 120] (v6);
\draw[fermion] (v6) to[out = 240, in = 300] (v5);
\end{tikzpicture}
}
+ \cdots\\
\Sigma_{\text{TMA}} =
\scalebox{.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[below = of v1](f1);
\draw[photon](v1) -- (f1);
\draw[fermion] (v1) arc (-90:270:0.6cm);
\end{tikzpicture}
}
+&
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, below = of v2] (v3);
\coordinate[vertex, left = of v3] (v4);
\draw[photon](v1) -- (v4);
\draw[photon](v2) -- (v3);
\draw[fermion] (v4) -- (v3);
\draw[fermion] (v2) to [out = 120, in = 60] (v1);
\draw[fermion] (v1) to [out = 300, in = 240] (v2);
\end{tikzpicture}
}
+
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, right = of v2] (v3);
\coordinate[vertex, below = of v3] (v4);
\coordinate[vertex, below = of v2] (v5);
\coordinate[vertex, below = of v1] (v6);
\draw[photon](v1) -- (v6);
\draw[photon](v2) -- (v5);
\draw[photon](v3) -- (v4);
\draw[fermion] (v1) -- (v2);
\draw[fermion] (v2) -- (v3);
\draw[fermion] (v5) -- (v4);
\draw[fermion] (v6) -- (v5);
\draw[fermion] (v3) to[out = 120, in = 60] (v1);
\end{tikzpicture}
}
+ \cdots \\
\Sigma_{\text{FLEX}} =
\scalebox{.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[below = of v1](f1);
\draw[photon](v1) -- (f1);
\draw[fermion] (v1) arc (-90:270:0.6cm);
\end{tikzpicture}
}
+&
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, below = of v2] (v3);
\coordinate[vertex, left = of v3] (v4);
\draw[photon](v1) -- (v4);
\draw[photon](v2) -- (v3);
\draw[fermion] (v4) -- (v3);
\draw[fermion] (v1) to [out = 60, in = 120] (v2);
\draw[fermion] (v2) to [out = 240, in = 300] (v1);
\end{tikzpicture}
}
+
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, above = of v2] (v3);
\coordinate[vertex, right = of v3] (v4);
\coordinate[vertex, below = of v4] (v5);
\coordinate[vertex, right = of v5] (v6);
\coordinate[vertex, below = of v6] (v7);
\coordinate[vertex, below = of v1] (v8);
\draw[photon](v1) -- (v8);
\draw[photon](v2) -- (v3);
\draw[photon](v4) -- (v5);
\draw[photon](v6) -- (v7);
\draw[fermion] (v8) -- (v7);
\draw[fermion] (v1) to[out = 60, in = 120] (v2);
\draw[fermion] (v2) to[out = 240, in = 300] (v1);
\draw[fermion] (v3) to[out = 60, in = 120] (v4);
\draw[fermion] (v4) to[out = 240, in = 300] (v3);
\draw[fermion] (v5) to[out = 60, in = 120] (v6);
\draw[fermion] (v6) to[out = 240, in = 300] (v5);
\end{tikzpicture}
}
+ \cdots\\
+& 
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, right = of v2] (v3);
\coordinate[vertex, below = of v3] (v4);
\coordinate[vertex, below = of v2] (v5);
\coordinate[vertex, below = of v1] (v6);
\draw[photon](v1) -- (v6);
\draw[photon](v2) -- (v5);
\draw[photon](v3) -- (v4);
\draw[fermion] (v2) -- (v1);
\draw[fermion] (v3) -- (v2);
\draw[fermion] (v5) -- (v4);
\draw[fermion] (v6) -- (v5);
\draw[fermion] (v1) to[out = 60, in = 120] (v3);
\end{tikzpicture}
}
+
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, right = of v2] (v3);
\coordinate[vertex, right = of v3] (v4);
\coordinate[vertex, below = of v4] (v5);
\coordinate[vertex, below = of v3] (v6);
\coordinate[vertex, below = of v2] (v7);
\coordinate[vertex, below = of v1] (v8);
\draw[photon](v1) -- (v8);
\draw[photon](v2) -- (v7);
\draw[photon](v3) -- (v6);
\draw[photon](v4) -- (v5);
\draw[fermion] (v2) -- (v1);
\draw[fermion] (v3) -- (v2);
\draw[fermion] (v4) -- (v3);
\draw[fermion] (v6) -- (v5);
\draw[fermion] (v7) -- (v6);
\draw[fermion] (v8) -- (v7);
\draw[fermion] (v1) to[out = 60, in = 120] (v4);
\end{tikzpicture}
}
+ \cdots\\
+& 
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, right = of v2] (v3);
\coordinate[vertex, below = of v3] (v4);
\coordinate[vertex, below = of v2] (v5);
\coordinate[vertex, below = of v1] (v6);
\draw[photon](v1) -- (v6);
\draw[photon](v2) -- (v5);
\draw[photon](v3) -- (v4);
\draw[fermion] (v1) -- (v2);
\draw[fermion] (v2) -- (v3);
\draw[fermion] (v5) -- (v4);
\draw[fermion] (v6) -- (v5);
\draw[fermion] (v3) to[out = 120, in = 60] (v1);
\end{tikzpicture}
}
+
\scalebox{0.6}{
\begin{tikzpicture}[node distance=1.2cm and 1.2cm]
\coordinate[vertex] (v1);
\coordinate[vertex, right = of v1] (v2);
\coordinate[vertex, right = of v2] (v3);
\coordinate[vertex, right = of v3] (v4);
\coordinate[vertex, below = of v4] (v5);
\coordinate[vertex, below = of v3] (v6);
\coordinate[vertex, below = of v2] (v7);
\coordinate[vertex, below = of v1] (v8);
\draw[photon](v1) -- (v8);
\draw[photon](v2) -- (v7);
\draw[photon](v3) -- (v6);
\draw[photon](v4) -- (v5);
\draw[fermion] (v1) -- (v2);
\draw[fermion] (v2) -- (v3);
\draw[fermion] (v3) -- (v4);
\draw[fermion] (v6) -- (v5);
\draw[fermion] (v7) -- (v6);
\draw[fermion] (v8) -- (v7);
\draw[fermion] (v4) to[out = 120, in = 60] (v1);
\end{tikzpicture}
}
+ \cdots
\end{align*}
\end{minipage}
\endpgfgraphicnamed

